Non-neural Models Matter: A Re-evaluation of Neural Referring Expression Generation Systems

In recent years, neural models have often outperformed rule-based and classic Machine Learning approaches in NLG. These classic approaches are now often disregarded, for example when new neural models are evaluated. We argue that they should not be overlooked, since, for some tasks, well-designed non-neural approaches achieve better performance than neural ones. In this paper, the task of generating referring expressions in linguistic context is used as an example. We examined two very different English datasets (WEBNLG and WSJ), and evaluated each algorithm using both automatic and human evaluations. Overall, the results of these evaluations suggest that rule-based systems with simple rule sets achieve on-par or better performance on both datasets compared to state-of-the-art neural REG systems. In the case of the more realistic dataset, WSJ, a machine learning-based system with well-designed linguistic features performed best. We hope that our work can encourage researchers to consider non-neural models in future.

==> tab/access.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lp{13cm}}
\toprule
Model & Input Text \\ \midrule
Neural Models & \underline{AWH\_Engineering\_College} is in \underline{``Kuttikkattoor''} , \underline{India} in the state of \underline{Kerala} . \underline{AWH\_Engineering\_College} has 250 employees and \underline{Kerala} is ruled by \underline{Kochi} . The \textbf{\underline{Ganges}} River is also found in \underline{India} . \\
\midrule
Rule Based Models & \underline{AWH\_Engineering\_College} has 250 employees and \underline{Kerala} is ruled by \underline{Kochi} . The \textbf{\underline{Ganges}} River is also found in \underline{India} . \\ \midrule
ML Based Models & \underline{AWH\_Engineering\_College} is in \underline{``Kuttikkattoor''} , \underline{India} in the state of \underline{Kerala} . \underline{AWH\_Engineering\_College} has 250 employees and \underline{Kerala} is ruled by \underline{Kochi} . The \textbf{\underline{Ganges}} River is also found in \underline{India} . \\
\bottomrule
\end{tabular}
\caption{A example data from the \textsc{webnlg} corpus. In the delexicalised text, every entity is \underline{underlined}, the target entity is \textbf{boldfaced}, the pre-context is coloured in \textcolor{blue}{blue}, and the pos-context is coloured in \textcolor{green}{green}.}
\label{tab:sample}
\end{table*}

==> tab/feat_ML_L.tex <==
\begin{table*}[b]
\small
% \begin{tabular}{ll}
% \toprule
% Feature type & Definition \\ \midrule
% \texttt{Grammatical Role} & Grammatical Role of $r$   \\
% \texttt{Grammatical Role} &  Grammatical Role of the antecedent \\
% \texttt{Inherent features} & Entity type (e.g. human, city, country, organization)  \\
% \texttt{Inherent features} & Plurality: Is $r$ plural or singular? (only \textsc{wsj})   \\
% \texttt{Inherent feature} & Gender \\
% \texttt{Recency} & categorical distance between $r$ and its antecedent in number of \texttt{words}\\
% \texttt{Recency} & categorical distance between $r$ and its antecedent in number of \texttt{sentences}\\
% \texttt{Recency} & categorical distance between $r$ and its antecedent in number of \texttt{paragraphs} (only \textsc{wsj})\\
% \bottomrule
% \end{tabular}
% \caption{Features used in the \textsc{webnlg} and \textsc{wsj} ML-L systems. Each feature is defined and calculated for each target entity $r$. \texttt{Antecedent} refers to the first co-referential referring expressions preceding the current $r$.}
% \label{tab:ml-l-feat}
\begin{tabular}{ll}
\toprule
Feature Class & Definition \\ \midrule
\texttt{Grammatical Role} & Grammatical Role of $r$   \\
\texttt{Grammatical Role} &  Grammatical Role of the antecedent \\
\texttt{Meta information} & Entity type (e.g. human, city, country, organization)  \\
\texttt{Meta information} & Plurality: Is $r$ plural or singular? (only \textsc{wsj})   \\
\texttt{Meta information} & Gender \\
\texttt{Recency} & Categorical distance between $r$ and its antecedent in number of \texttt{words}\\
\texttt{Recency} & Categorical distance between $r$ and its antecedent in number of \texttt{sentences}\\
\texttt{Recency} & Categorical distance between $r$ and its antecedent in number of \texttt{paragraphs} (only \textsc{wsj})\\
\bottomrule
\end{tabular}
\caption{Features used in the \texttt{ML-L} models. }
\label{tab:ml-l-feat}
\end{table*}



==> tab/webnlg.tex <==
\begin{table*}[t!]
\small
\centering
\begin{tabular}{p{15cm}}
\toprule
\textbf{Triples}: \\
AWH\_Engineering\_College | country | India \\
Kerala | leaderName | Kochi \\
AWH\_Engineering\_College | academicStaffSize | 250 \\
AWH\_Engineering\_College | state | Kerala \\
AWH\_Engineering\_College | city | ``Kuttikkattoor'' \\
India | river | Ganges \\
\midrule
\textbf{Text}: AWH Engineering College is in Kuttikkattoor, India in the state of Kerala. The school has 250 employees and Kerala is ruled by Kochi. The Ganges River is also found in India. \\
\textbf{Delexicialised Text}: \textcolor{blue}{\underline{AWH\_Engineering\_College} is in \underline{``Kuttikkattoor''} , \underline{India} in the state of \underline{Kerala} . }\textbf{\underline{AWH\_Engineering\_College}} \textcolor{ForestGreen}{has 250 employees and \underline{Kerala} is ruled by \underline{Kochi} . The \underline{Ganges} River is also found in \underline{India} .}\\
\bottomrule
\end{tabular}
\caption{An example data from the \textsc{webnlg} corpus. In the delexicalised text, every entity is \underline{underlined}, the target entity is \textbf{boldfaced}, the pre-context is coloured in \textcolor{blue}{blue}, and the pos-context is coloured in \textcolor{ForestGreen}{green}.}
\label{tab:sample}
\end{table*}

==> tab/wsj_delex.tex <==
\begin{table*}[ht]
\small
\centering
\scalebox{1}{
\begin{tabular}{p{15cm}}
\toprule
\textbf{Text}: The presence of Unilever and P\&G is likely to increase the impact of advertising on cosmetics . While the two are among the world 's biggest advertisers , most makers of upscale cosmetics spend relatively little on national ads . Instead , they  focus on events in department stores and pour their  promotional budgets into gifts that go along with purchases . Estee Lauder , for example , spends only an estimated 5 \% of sales on advertising in the U.S. , and Mr. Lauder says he  has no plans to change his  strategy . The most dramatic changes , however , probably will come in new - product development . \\ \midrule
\textbf{Delexicialized Text}: \\
\vspace{0.02cm}
\textbf{Pre-context}: The presence of \underline{P\&G\_and\_Unilever} is likely to increase the impact of advertising on cosmetics . While \underline{P\&G\_and\_Unilever} are among the world 's biggest advertisers , \underline{most\_makers\_of\_upscale\_cosmetics} spend relatively little on national ads . Instead ,\\
\vspace{0.02cm}
\textbf{Target Entity}: \underline{most\_makers\_of\_upscale\_cosmetics}\\
\vspace{0.02cm}
\textbf{Post-context}: focus on events in department stores and pour \underline{most\_makers\_of\_upscale\_cosmetics} promotional budgets into gifts that go along with purchases . \underline{Estee\_Lauder} , for example , spends only an estimated 5 \% of sales on advertising in the U.S. , and \underline{Mr.\_Lauder} says \underline{Mr.\_Lauder} has no plans to change \underline{Mr.\_Lauder} strategy . The most dramatic changes , however , probably will come in new-product development .\\
\bottomrule
\end{tabular}}
\caption[An example data from the \textsc{WSJ} corpus.]{An example data from the WSJ corpus. In the delexicalized text, every entity is \underline{underlined}.}
\label{tab:wsjsample}
\end{table*}

==> tab/wsj_minidoc.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lccccccc}
\toprule
Model & RE Acc.$\uparrow$ & SED$\downarrow$ & BLEU$\uparrow$ & Text Acc.$\uparrow$ & Precision$\uparrow$ & Recall$\uparrow$ & F1$\uparrow$ \\ \midrule
\texttt{RREG-S} & \underline{41.77} & \underline{12.27} & \underline{80.67} & 3.05 & 66.97 & 63.76 & 64.84 \\
\texttt{RREG-L} & 39.11 & 12.69 & 80.60 & \underline{3.32} & 66.22 & 58.36 & 59.06 \\
\texttt{Feat-S} & 34.93 & 15.01 & 79.26 & 2.22 & \underline{78.39} & 64.19 & 66.66 \\
\texttt{Feat-L} & \textbf{53.00} & \textbf{11.22} & \textbf{82.83} & \textbf{6.65} & \textbf{82.61} & \textbf{83.72} & \textbf{83.14} \\
\texttt{ATT+Copy} & 38.71 & 13.89 & 79.48 & \underline{3.32} & 72.56 & \underline{70.65} & \underline{71.48} \\
\texttt{ATT+Meta} & 38.43 & 12.45 & 79.20 & \underline{3.32} & 71.12 & 70.41 & 70.74 \\
\bottomrule
\end{tabular}
\caption{Automatic Evaluation Results on mini-doc splitted \textsc{wsj}.}
\label{tab:wsj_minidoc}
\end{table*}
